AFFSegNet: Adaptive Feature Fusion Segmentation Network for Microtumors and Multi-Organ Segmentation

Medical image segmentation, a crucial task in computer vision, facilitates the automated delineation of anatomical structures and pathologies, supporting clinicians in diagnosis, treatment planning, and disease monitoring. Notably, transformers employing shifted window-based self-attention have demonstrated exceptional performance. However, their reliance on local window attention limits the fusion of local and global contextual information, crucial for segmenting microtumors and miniature organs. To address this limitation, we propose the Adaptive Semantic Segmentation Network (ASSNet), a transformer architecture that effectively integrates local and global features for precise medical image segmentation. ASSNet comprises a transformer-based U-shaped encoder-decoder network. The encoder utilizes shifted window self-attention across five resolutions to extract multi-scale features, which are then propagated to the decoder through skip connections. We introduce an augmented multi-layer perceptron within the encoder to explicitly model long-range dependencies during feature extraction. Recognizing the constraints of conventional symmetrical encoder-decoder designs, we propose an Adaptive Feature Fusion (AFF) decoder to complement our encoder. This decoder incorporates three key components: the Long Range Dependencies (LRD) block, the Multi-Scale Feature Fusion (MFF) block, and the Adaptive Semantic Center (ASC) block. These components synergistically facilitate the effective fusion of multi-scale features extracted by the decoder while capturing long-range dependencies and refining object boundaries. Comprehensive experiments on diverse medical image segmentation tasks, including multi-organ, liver tumor, and bladder tumor segmentation, demonstrate that ASSNet achieves state-of-the-art results. Code and models are available at: \url{https://github.com/lzeeorno/ASSNet}.

==> figtex/fig5.tex <==
% \begin{figure}[h]
% \centerline{\includegraphics[width=\columnwidth]{figs/ISICDM2019Result.png}}
% \caption{ISICDM2019 Segmentation Result}
% \label{fig5}
% \end{figure}

\begin{figure}[ht]
\begin{tikzpicture}[%
  spy using outlines = {rectangle,
                        magnification=2,
                        connect spies}]

  % 载入图像(注意定位锚点为西南，即左下角)
  \node[anchor=south west, inner sep=0] (img1) at (0,0)
  {\includegraphics[width=\columnwidth]{figs/ISICDM2019_PrecSegNet_Result.pdf}};

  % 限定坐标区域
  \begin{scope}[x={(img1.south east)}, y={(img1.north west)}]
    % 绘制坐标辅助网络
    % \drawgrid

    % 第1列
    \coordinate (spypoint) at (0.29, 0.775);
    \coordinate (magnifyglass) at (0.18,0.91);
    % 第2个放大镜锚点
    \coordinate (spypoint2) at (0.3, 0.545);
    \coordinate (magnifyglass2) at (0.18, 0.68);
    % 第3个放大镜锚点
    \coordinate (spypoint3) at (0.3, 0.31);
    \coordinate (magnifyglass3) at (0.18, 0.45);
    % 第4个放大镜锚点
    \coordinate (spypoint4) at (0.31, 0.09);
    \coordinate (magnifyglass4) at (0.18, 0.225);

    % 第2列
    \coordinate (spypoint5) at (0.41, 0.86);
    \coordinate (magnifyglass5) at (0.345, 0.91);
    % 第2个放大镜锚点
    \coordinate (spypoint6) at (0.41, 0.636);
    \coordinate (magnifyglass6) at (0.345, 0.68);
    % 第3个放大镜锚点
    \coordinate (spypoint7) at (0.416, 0.39);
    \coordinate (magnifyglass7) at (0.345, 0.45);
    % 第4个放大镜锚点
    \coordinate (spypoint8) at (0.41, 0.17);
    \coordinate (magnifyglass8) at (0.345, 0.225);

    % 第3列
    \coordinate (spypoint9) at (0.59, 0.77);
    \coordinate (magnifyglass9) at (0.51, 0.91);
    % 第2个放大镜锚点
    \coordinate (spypoint10) at (0.59, 0.53);
    \coordinate (magnifyglass10) at (0.51, 0.68);
    % 第3个放大镜锚点
    \coordinate (spypoint11) at (0.59, 0.3);
    \coordinate (magnifyglass11) at (0.51, 0.45);
    % 第4个放大镜锚点
    \coordinate (spypoint12) at (0.585, 0.085);
    \coordinate (magnifyglass12) at (0.51, 0.225);

    % 第4列
    \coordinate (spypoint13) at (0.73, 0.73);
    \coordinate (magnifyglass13) at (0.675, 0.91);
    % 第2个放大镜锚点
    \coordinate (spypoint14) at (0.73, 0.50);
    \coordinate (magnifyglass14) at (0.675, 0.68);
    % 第3个放大镜锚点
    \coordinate (spypoint15) at (0.725, 0.28);
    \coordinate (magnifyglass15) at (0.675, 0.45);
    % 第4个放大镜锚点
    \coordinate (spypoint16) at (0.725, 0.045);
    \coordinate (magnifyglass16) at (0.675, 0.225);

    % 第5列
    \coordinate (spypoint17) at (0.885, 0.75);
    \coordinate (magnifyglass17) at (0.84, 0.91);
    % 第2个放大镜锚点
    \coordinate (spypoint18) at (0.88, 0.53);
    \coordinate (magnifyglass18) at (0.84, 0.68);
    % 第3个放大镜锚点
    \coordinate (spypoint19) at (0.89, 0.29);
    \coordinate (magnifyglass19) at (0.84, 0.45);
    % 第4个放大镜锚点
    \coordinate (spypoint20) at (0.895, 0.07);
    \coordinate (magnifyglass20) at (0.84, 0.225);
    
    \end{scope}

    \spy[anchor=north west, white, size=0.5cm, very thick] on (spypoint) in node[fill=white] at (magnifyglass);
    \spy[anchor=north west, white, size=0.5cm, very thick] on (spypoint2) in node[fill=white] at (magnifyglass2);
    \spy[anchor=north west, white, size=0.5cm, very thick] on (spypoint3) in node[fill=white] at (magnifyglass3);
    \spy[anchor=north west, white, size=0.5cm, very thick] on (spypoint4) in node[fill=white] at (magnifyglass4);

    \spy[anchor=north west, white, size=0.5cm, very thick] on (spypoint5) in node[fill=white] at (magnifyglass5);
    \spy[anchor=north west, white, size=0.5cm, very thick] on (spypoint6) in node[fill=white] at (magnifyglass6);
    \spy[anchor=north west, white, size=0.5cm, very thick] on (spypoint7) in node[fill=white] at (magnifyglass7);
    \spy[anchor=north west, white, size=0.5cm, very thick] on (spypoint8) in node[fill=white] at (magnifyglass8);

    \spy[anchor=north west, white, size=0.5cm, very thick] on (spypoint9) in node[fill=white] at (magnifyglass9);
    \spy[anchor=north west, white, size=0.5cm, very thick] on (spypoint10) in node[fill=white] at (magnifyglass10);
    \spy[anchor=north west, white, size=0.5cm, very thick] on (spypoint11) in node[fill=white] at (magnifyglass11);
    \spy[anchor=north west, white, size=0.5cm, very thick] on (spypoint12) in node[fill=white] at (magnifyglass12);

    \spy[anchor=north west, white, size=0.5cm, very thick,width=1.2cm, height=0.5cm] on (spypoint13) in node[fill=white] at (magnifyglass13);
    \spy[anchor=north west, white, size=0.5cm, very thick,width=1.2cm, height=0.5cm] on (spypoint14) in node[fill=white] at (magnifyglass14);
    \spy[anchor=north west, white, size=0.5cm, very thick,width=1.2cm, height=0.5cm] on (spypoint15) in node[fill=white] at (magnifyglass15);
    \spy[anchor=north west, white, size=0.5cm, very thick,width=1.2cm, height=0.5cm] on (spypoint16) in node[fill=white] at (magnifyglass16);

    \spy[anchor=north west, white, size=0.5cm, very thick] on (spypoint17) in node[fill=white] at (magnifyglass17);
    \spy[anchor=north west, white, size=0.5cm, very thick] on (spypoint18) in node[fill=white] at (magnifyglass18);
    \spy[anchor=north west, white, size=0.5cm, very thick] on (spypoint19) in node[fill=white] at (magnifyglass19);
    \spy[anchor=north west, white, size=0.5cm, very thick] on (spypoint20) in node[fill=white] at (magnifyglass20);

\end{tikzpicture}
\caption{ISICDM2019 Prediction Result.}
\label{fig5}
\end{figure}

==> figtex/fig6.tex <==
\begin{figure}[ht]
\begin{tikzpicture}[%
  spy using outlines = {rectangle,
                        magnification=2,
                        connect spies}]

  % 载入图像(注意定位锚点为西南，即左下角)
  \node[anchor=south west, inner sep=0] (img1) at (0,0)
  {\includegraphics[width=\columnwidth]{figs/Synapse_PrecSegNet_Result.pdf}};

  % 限定坐标区域
  \begin{scope}[x={(img1.south east)}, y={(img1.north west)}]
    % 绘制坐标辅助网络
    % \drawgrid

    % 第1列
    \coordinate (spypoint) at (0.3, 0.72);
    \coordinate (magnifyglass) at (0.197,0.879);
    % 第2个放大镜锚点
    \coordinate (spypoint2) at (0.305, 0.49);
    \coordinate (magnifyglass2) at (0.197, 0.66);
    % 第3个放大镜锚点
    \coordinate (spypoint3) at (0.3, 0.28);
    \coordinate (magnifyglass3) at (0.197, 0.44);


    % 第2列
    \coordinate (spypoint5) at (0.42, 0.76);
    \coordinate (magnifyglass5) at (0.358, 0.879);
    % 第2个放大镜锚点
    \coordinate (spypoint6) at (0.42, 0.54);
    \coordinate (magnifyglass6) at (0.358, 0.66);
    % 第3个放大镜锚点
    \coordinate (spypoint7) at (0.42, 0.33);
    \coordinate (magnifyglass7) at (0.358, 0.44);


    % 第3列
    \coordinate (spypoint9) at (0.635, 0.8);
    \coordinate (magnifyglass9) at (0.52, 0.879);
    % 第2个放大镜锚点
    \coordinate (spypoint10) at (0.635, 0.58);
    \coordinate (magnifyglass10) at (0.52, 0.66);
    % 第3个放大镜锚点
    \coordinate (spypoint11) at (0.635, 0.36);
    \coordinate (magnifyglass11) at (0.52, 0.44);


    % 第4列
    \coordinate (spypoint13) at (0.77, 0.825);
    \coordinate (magnifyglass13) at (0.68, 0.879);
    % 第2个放大镜锚点
    \coordinate (spypoint14) at (0.77, 0.6);
    \coordinate (magnifyglass14) at (0.68, 0.66);
    % 第3个放大镜锚点
    \coordinate (spypoint15) at (0.77, 0.38);
    \coordinate (magnifyglass15) at (0.68, 0.44);


    % 第5列
    \coordinate (spypoint17) at (0.94, 0.72);
    \coordinate (magnifyglass17) at (0.84, 0.879);
    % 第2个放大镜锚点
    \coordinate (spypoint18) at (0.94, 0.51);
    \coordinate (magnifyglass18) at (0.84, 0.66);
    % 第3个放大镜锚点
    \coordinate (spypoint19) at (0.94, 0.29);
    \coordinate (magnifyglass19) at (0.84, 0.44);

    
    \end{scope}

    \spy[anchor=north west, white, size=0.5cm, very thick] on (spypoint) in node[fill=white] at (magnifyglass);
    \spy[anchor=north west, white, size=0.5cm, very thick] on (spypoint2) in node[fill=white] at (magnifyglass2);
    \spy[anchor=north west, white, size=0.5cm, very thick] on (spypoint3) in node[fill=white] at (magnifyglass3);


    \spy[anchor=north west, white, size=0.5cm, very thick] on (spypoint5) in node[fill=white] at (magnifyglass5);
    \spy[anchor=north west, white, size=0.5cm, very thick] on (spypoint6) in node[fill=white] at (magnifyglass6);
    \spy[anchor=north west, white, size=0.5cm, very thick] on (spypoint7) in node[fill=white] at (magnifyglass7);


    \spy[anchor=north west, white, size=0.5cm, very thick] on (spypoint9) in node[fill=white] at (magnifyglass9);
    \spy[anchor=north west, white, size=0.5cm, very thick] on (spypoint10) in node[fill=white] at (magnifyglass10);
    \spy[anchor=north west, white, size=0.5cm, very thick] on (spypoint11) in node[fill=white] at (magnifyglass11);


    \spy[anchor=north west, white, size=0.5cm, very thick, height=0.7cm] on (spypoint13) in node[fill=white] at (magnifyglass13);
    \spy[anchor=north west, white, size=0.5cm, very thick, height=0.7cm] on (spypoint14) in node[fill=white] at (magnifyglass14);
    \spy[anchor=north west, white, size=0.5cm, very thick, height=0.7cm] on (spypoint15) in node[fill=white] at (magnifyglass15);


    \spy[anchor=north west, white, size=0.5cm, very thick] on (spypoint17) in node[fill=white] at (magnifyglass17);
    \spy[anchor=north west, white, size=0.5cm, very thick] on (spypoint18) in node[fill=white] at (magnifyglass18);
    \spy[anchor=north west, white, size=0.5cm, very thick] on (spypoint19) in node[fill=white] at (magnifyglass19);


\end{tikzpicture}
\caption{Synapse Prediction Result.}
\label{fig6}
\end{figure}

==> theorem/theorem1.tex <==
\begin{algorithm}[H]
\caption{SMAFormer Algorithm}
\label{alg:smaformer}
\begin{algorithmic}[1]
\Require Image $x$
\Ensure Segmentation Map $\hat{y}$ 

\State $x_1 = \text{ReLU}(\text{BatchNorm}(Conv_{3\times3}(x)))$ \Comment{Initial Convolution}
\State $x_1 = x_1 + Conv_{3\times3}(x)$ \Comment{Input Skip Connection}

\For{$i = 1$ to $5$}
    \State $x_i = \text{MaxPool}(x_i)$ \Comment{Max Pooling}
    \State $x_{i+1} = \text{ResidualConv}(x_i)$ \Comment{Residual Convolution Block}
\EndFor

\State $e_1 = \text{Modulator}(x_1)$ \Comment{Patch Embedding 1}
\State $e_1 = \text{reshape}(e_1)$ \Comment{Reshape for Transformer}
\State $e_1 = \text{EncoderBlock}(e_1)$ \Comment{Encoder Block 1}

\For{$i = 2$ to $6$}
    \State $e_i = \text{Modulator}(x_i)$ \Comment{Patch Embedding}
    \State $e_i = \text{reshape}(e_i)$ \Comment{Reshape for Transformer}
    \State $e_i = \text{EncoderBlock}(e_i, e_{i-1})$ \Comment{Encoder Block}
\EndFor

\State $d_6 = e_6$ \Comment{Initialize Decoder}

\For{$i = 5$ to $1$}
    \State $d_i = \text{Upsample}(d_{i+1})$ \Comment{Upsampling}
    \State $d_i = \text{DecoderBlock}(d_i, e_i)$ \Comment{Decoder Block}
    \State $attn = \text{Cross\_AttentionBlock}(x_i, d_i)$ \Comment{Cross Attention}
    \State $d_i = attn * d_i$ \Comment{Attention Refinement}
\EndFor

\State $\hat{y} = \text{Conv}_{1\times1}(\text{Upsample}(d_1))$ \Comment{Final Output}
\end{algorithmic}
\end{algorithm}
